The Solar Neutrino Problem and Solar Neutrino Oscillations in Vacuum and in Matter

The solar neutrino problem is reviewed and the possible vacuum oscillation and MSW solutions of the problem are considered.

==> schladf97.tex <==
\magnification 1200
\def\dm{$\Delta m^2$\hskip 0.2cm }
\def\dmf{\Delta m^2}
\def\sn{$\sin^2 2\theta$\hskip 0.2cm }
\def\snf{\sin^2 2\theta}
\def\trna{$\nu_e \rightarrow \nu_a$}
\def\trnm{$\nu_e \rightarrow \nu_{\mu}$}
\def\trns{$\nu_e \rightarrow \nu_s$}
\line{\hfill Ref. SISSA 30/98/EP}
\vskip 2cm
\centerline{\bf THE SOLAR NEUTRINO PROBLEM AND SOLAR NEUTRINO OSCILLATIONS}
\centerline{\bf IN VACUUM AND IN MATTER}
\centerline{\bf }
\vskip 1cm
\centerline{S.T. Petcov
\footnote{*}
 {\rm Lectures given at the 36 International School on Nuclear
and Particle Physics, 
          March 1 - 8, 1997, Schladming, Austria; to be
   published in the Proceedings of the School.}  
{}\footnote{$^\dagger$}
 {Also at: Institute of Nuclear Research and Nuclear Energy,
Bulgarian Academy of Sciences, BG-1784 Sofia,
Bulgaria.}}
\centerline{Scuola
 Internazionale Superiore di Studi Avanzati,}
\centerline{and Istituto Nazionale di Fisica Nucleare,
                       Sezione di Trieste,}
\centerline{I-34013 Trieste, Italy}
\vskip 2cm
\centerline{\bf Abstract}
\vskip 0.3cm
The solar neutrino problem is reviewed and the possible vacuum oscillation
and MSW solutions of the problem are considered. 
\vskip 2.5cm
Ref. SISSA 30/98/EP 

March, 1998.
\footline={\hfil}
\eject
\bye
 





